Security-Aware Sensor Fusion with MATE: the Multi-Agent Trust Estimator

Lacking security awareness, sensor fusion in systems with multi-agent networks such as smart cities is vulnerable to attacks. To guard against recent threats, we design security-aware sensor fusion that is based on the estimates of distributions over trust. Trust estimation can be cast as a hidden Markov model, and we solve it by mapping sensor data to trust pseudomeasurements (PSMs) that recursively update trust posteriors in a Bayesian context. Trust then feeds sensor fusion to facilitate trust-weighted updates to situational awareness. Essential to security-awareness are a novel field of view estimator, logic to map sensor data into PSMs, and the derivation of efficient Bayesian updates. We evaluate security-aware fusion under attacks on agents using case studies and Monte Carlo simulation in the physics-based Unreal Engine simulator, CARLA. A mix of novel and classical security-relevant metrics show that our security-aware fusion enables building trustworthy situational awareness even in hostile conditions.

==> figures/figure_fusion_algorithms.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{example-image-a}
    \caption{Multi-agent fusion algorithms for collaborative state estimation.}
    \label{fig:fusion-algorithms}
\end{figure}

==> figures/figure_fusion_smart_city.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{diagrams/fusion_smart_city.png}
    \caption{Advances in sensing, networking, and computing are fueling \emph{smart cities} that boast the interconnectedness of heterogeneous agents. Trusted computing centers can check for inter-agent consistency to flag compromised data and secure safety-critical domains such as urban intersections.}
    \label{fig:smart-city}
\end{figure}

==> figures/figure_results_mc_tuning.tex <==
% [trim={left bottom right top},clip]
\begin{figure}[t]
    \centering
    \includegraphics[trim={0cm 2cm 0cm 0cm},clip,width=0.8\linewidth]{diagrams/trust_tune_agent_negativity_bias_median.pdf}
    \caption{Tuning is performed systematically over parameters with randomized adversarial datasets. Here, a sample outcome of tuning the negativity bias parameter (see Eq.~\ref{eq:beta-bernoulli-update-weighted}) of the trust algorithm with 100 bias options on over 100 Monte Carlo-generated adversarial datasets at 600 frames yields nearly 6 million metric datapoints. Color denotes different metrics (see Sec.~\ref{sec:exp-ue-metrics}). Shown with varying opacity lines are the percentiles from 10-90 over the trials of the median over the frames. An objective function over metrics directs the tuning process. Clearly, increasing the agent's negativity bias parameter improves the agent's trust distribution metric.}
    \label{fig:results-mc-tuning}
\end{figure}

==> figures/figure_results_mc_tuning_all.tex <==
\begin{figure*}[t]
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Median outcome
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{diagrams/mc_tuning/trust_tune_agent_negativity_bias_median.pdf}
        \caption{Median ($Q=0.5$) metrics}
    \end{subfigure}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Two sigma below outcome
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{diagrams/mc_tuning/trust_tune_agent_negativity_bias_twosigmabelow.pdf}
        \caption{$2\sigma$ below median ($Q=0.025$) metrics}
    \end{subfigure}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Two dimensional surface
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{diagrams/mc_tuning/trust_tune_agent_negativity_bias_twosigmabelow.pdf}
        \caption{$2\sigma$ below median ($Q=0.025$) metrics}
    \end{subfigure}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caption{Caption}
    \label{fig:results-mc-tuning}
\end{figure*}

==> tables/table_threat_model.tex <==
% \begin{table}
% % Table 1: Manifest
% \parbox{.45\linewidth}{
%     \centering
%     \begin{tabular}{p{4cm}}
%     \textbf{Manifest Characteristic} \\
%     \toprule
%     \emph{False positive:} Fake object(s) are injected into the perception. \\
%     \emph{False negative:} Existing object(s) are removed from perception. \\
%     \emph{Translation:} Detections are translated spatially. \\
%     \emph{Pose Error:} Agent transmits compromised ownship pose.
%     \end{tabular}
%     \caption{Foo}
%     \label{tab:threat-model-manifest}
% }
% %
% \hfill
% %
% % Table 2: Temporal
% \parbox{.45\linewidth}{
%     \centering
%     \begin{tabular}{p{4cm}}
%     \textbf{Temporal Characteristic} \\
%     \toprule
%     \emph{Static:} Threat is temporally-invariant, e.g.,~spatially-fixed. \\
%     \emph{Markovian:} Threat evolves with random walk dynamics over time. \\
%     \emph{Trajectory/Object:} Threat demonstrates a predefined trajectory or consistently targets a particular object in the scene.
%     \end{tabular}
%     \caption{Bar}
%     \label{tab:threat-model-temporal}
% }
% \end{table}
